Local Descent For Temporal Logic Falsification of Cyber-Physical Systems (Extended Technical Report)

One way to analyze Cyber-Physical Systems is by modeling them as hybrid automata. Since reachability analysis for hybrid nonlinear automata is a very challenging and computationally expensive problem, in practice, engineers try to solve the requirements falsification problem. In one method, the falsification problem is solved by minimizing a robustness metric induced by the requirements. This optimization problem is usually a non-convex non-smooth problem that requires heuristic and analytical guidance to be solved. In this paper, functional gradient descent for hybrid systems is utilized for locally decreasing the robustness metric. The local descent method is combined with Simulated Annealing as a global optimization method to search for unsafe behaviors.

==> review.tex <==
We would like to thank the reviewers for their helpful comments and suggestions on the manuscript. We believe that the comments have highlighted important questions that can be answered in the text. The final version of the paper will definitely cover required modifications with respect to any typos, missing definitions, and explanations. In the following we have addressed the reviewers' concerns:

Firstly, although we understand the reviewers' viewpoint, we politely disagree that the paper does not have relevance to the conference. In principle, certain CPS should satisfy hard real-time requirements which extend beyond just schedulability and network delays. Sometimes the system dynamics are complex enough that simple real-time requirements such as “whenever a change in the mode is detected, then the pressure will stabilize in the safety region within 30ms for up to 100ms” are hard to analyze and verify. In this paper, we deal with these kinds of problems.

Secondly, the guarantees are on the convergence to a local minimum. The robustness value provides a neighborhood of safety or how close you are to falsification. Using a local upper bound on the dynamics it can be inferred whether it is possible to produce a falsifying behavior. See Abbas, et al CYBER 2014 on how probabilistic guarantees and confidence intervals can be derived.
 
Thirdly, we acknowledge that we should cite the related works [1][2][3] by Donze, et al. These works differ from our work from different aspects:
1. As mentioned by the reviewer all these works solve different problems using sensitivity analysis, [1] computes the sensitivity of the formula with respect to parameters in the predicates and [2] approximates reachable sets. Our manuscript, however, tries to solve a falsification problem.

2. In [1], the idea is to calculate the sensitivity of the temporal logic robustness function to parameters, while in the paper it is assumed that one can differentiate the predicates of this function with respect to parameters, generally the function and the predicates it consists of are nondifferentiable. To deal with this issue we tried to approach the problem differently: we calculate the sensitivity of the "trajectory" to the initial conditions and inputs and try to get it closer to the critical predicate (which does not have to be smooth or differentiable).

3. At the high level, unlike our method that considers general MTL formula, the problem in [2] is solved for safety properties without timing requirements.

4. Although "using the sensitivity analysis to solve the optimization falsification problem for hybrid systems" is the contribution we claim, not the sensitivity analysis itself, compared to [2], the analysis in our work is more general considering reset maps and is closer to the work in the paper entitled "Trajectory Sensitivity Analysis of Hybrid Systems", even though we believe that considering the hybrid systems as hybrid automata make the sensitivity analysis easier.

Finally, there were only a few papers related to falsification of hybrid systems like the reference [7] in the paper with which we could compare our method. However, the run-times reported there depend highly on system specs, parallelism, etc. and there were no results based on the number of simulations necessary for falsification. Furthermore, the run-times reported there is calculated after they find the sequence of locations that need to be met for falsification so they are hardly informative
